Submixing and Shift-invariant Stochastic Games

We consider zero-sum stochastic games with perfect information and finitely many states and actions. The payoff is computed by a function which associates to each infinite sequence of states and actions a real number. We prove that if the payoff function is both shift-invariant and submixing, then the game is half-positional, i.e. the first player has an optimal strategy which is both deterministic and stationary. This result relies on the existence of epsilon-subgame-perfect strategies in shift-invariant games, a second contribution of the paper. The techniques can be used to establish a third result: for shift-invariant and submixing payoff functions, the existence of finite-memory strategies for player 2 in one-player games implies the same property for two-player games as well.

==> subgameperfect.tex <==
\section{$\epsilon$-Subgame-Perfect Strategies}
\label{sec:subgameperfect}
The proof of \Cref{thm:main} hinges on a crucial property of games with perfect information, namely the fact that they admit $\epsilon$-subgame-perfect strategies, for all $\epsilon>0$. 
\begin{theorem}
  \label{thm:subgameperfect}
  Games equipped with a payoff function that is bounded and Borel-measurable, admit $\epsilon$-subgame-perfect strategies,
   for every $\epsilon>0$.
\end{theorem}
In this section we sketch the proof of this theorem, by giving a construction that takes some $\epsilon$-optimal strategy $\sigma$ and turns it into a $2\epsilon$-subgame-perfect strategy $\hat\sigma$. A full proof can be found in Mashiah-Yaakovi's paper \cite[Proposition 11]{correlated} in a more general setting, in the preprint version of the current paper \cite[Section 3]{preprintversion}, as well as in \cite{flesch2021subgame}.

The theorem is completely symmetric about the players, so it is sufficient to show that, say, the maximizer has $\epsilon$-subgame-perfect strategies. 

An $\epsilon$-optimal strategy $\sigma$ is a strategy that ensures (to within $\epsilon$) the largest payoff that it can be ensured from the starting position of the game. As the game progresses, if the adversary makes a non-optimal move at some point, that allows one to gain more, an $\epsilon$-optimal strategy does not necessarily take advantage of this slip up. The $\epsilon$-subgame-perfect strategies are that subset of strategies that do take advantage of any such non-optimal action of the adversary. How does one turn an $\epsilon$-optimal strategy to an $\epsilon$-subgame-perfect strategy? One simple observation suffices: if after the non-optimal action is played, $\sigma$ simply forgets the past, \ie resets its memory, then the payoff will be larger. We explain why the strategy that always resets the memory when the adversary has played a non-optimal action is $2\epsilon$-subgame-perfect. First, let us make this construction precise. 

A strategy $\sigma$ is not $2\epsilon$-subgame-perfect if and only if there exists some finite play $h:=s_0\cdots s_n$ such that
\begin{align}
  \label{eq:drop}
  \inf_\tau\ee {s_n}{\sigma[h],\tau}{f[h]} < \sup_{\sigma'}\inf_{\tau}\ee {s_n}{\sigma',\tau}{f[h]}-2\epsilon;
\end{align}
the reset strategy simply resets its memory when this happens. We give the formal definitions.
\begin{definition}
  \label{def:drop}The finite play $h:=s_0\cdots s_n$ is called a \emph{$(\epsilon,\sigma)$-drop} if \eqref{eq:drop} holds. We write
  \begin{align*}
    \Delta(\epsilon,\sigma)(h)\qquad\Leftrightarrow\qquad\text{h is a $(\epsilon,\sigma)$-drop}.
  \end{align*}
\end{definition}
It is plain that one can factorise any infinite play that has infinitely many drops,  into $h_1 h_2\cdots$ where each $h_i$ is a $(\epsilon,\sigma)$-drop, but no strict prefix of $h_i$ is $(\epsilon,\sigma)$-drop. For example:
\begin{center}
\includegraphics[width=.8\textwidth]{drops.pdf}
\end{center}
\begin{definition}
  We define the \emph{date} of the most recent (or latest) drop for all $s_0\cdots s_n$ inductively as:
  \begin{align*}
    \Lambda(\epsilon,\sigma)(s_0)&\defeq 0\\
    \Lambda(\epsilon,\sigma)(s_0\cdots s_n)&\defeq
    \begin{cases}
      n \qquad &\text{if $h$ is a $(\epsilon,\sigma)$-drop}\\
      \Lambda(\epsilon,\sigma)(s_0\cdots s_{n-1})\qquad &\text{otherwise},
    \end{cases}
  \end{align*}
  where
  \begin{align*}
    h\defeq s_{\ell}\cdots s_n,\ \ \ \text{and} \ \ \ \ell \defeq \Lambda(\epsilon,\sigma)(s_0\cdots s_{n-1}).
  \end{align*}
\end{definition}
The date of the most recent drop in the example above looks as follows:
\begin{center}
\includegraphics[width=.8\textwidth]{drops2.pdf}
\end{center}

The reset strategy resets its memory whenever a drop occurs, \ie it keeps the memory since the most recent drop:
\begin{definition}[Reset Strategy]\label{def:reset}
  For any strategy $\sigma$ we define the reset strategy $\reset\sigma$ as:
  \begin{align*}
    \reset\sigma(s_0\cdots s_n)=\sigma(s_\ell\cdots s_n),
  \end{align*}
  where
  \begin{align*}
    \ell\defeq\Lambda(\epsilon,\sigma)(s_0\cdots s_n).
  \end{align*}
\end{definition}
The crux of the proof of \Cref{thm:subgameperfect} is to show that under the strategy $\hat\sigma$ only finitely many resets occur, almost surely. Intuitively, this is because after every $(\epsilon,\sigma)$-drop, by resetting the memory, the maximizer gains at least some amount $\delta$ that is bounded away from zero. But it is not possible to gain infinitely many times $\delta$ because the payoff function is assumed to be bounded.

One way of formally proving this observation is to use martingale theory. We start with a strategy $\sigma$ that is $\epsilon$-optimal, and such that it only ever chooses actions that never decrease the value on average. Then one shows that only finitely many drops occur almost surely with the strategy $\hat\sigma$, and that furthermore the strategy $\hat\sigma$ is itself $\epsilon$-optimal. For the former, Doob's optional stopping theorem, and forward convergence theorem \cite[Theorem 11.5]{wiliamspr} are useful. Finally one proves:
\begin{lemma}\label{lem:subgame}
Let $\game$ be a game equipped with a shift-invariant payoff function.
Let $\epsilon \geq 0$ be a non-negative real number
and $\sigma$ be an $\epsilon$-optimal strategy in $\game$.
Then $\hat\sigma$ is $2\epsilon$-subgame-perfect in $\game$. 
\end{lemma}

The $\epsilon$-optimal strategies that we use, to turn into $2\epsilon$-subgame-perfect strategies $\hat\sigma$, are guaranteed to exist by Martin's theorem, \Cref{thm:martin}. 
%However, if in some game, one of the players, happens to have an optimal strategy (\ie a $0$-optimal strategy), then via the construction above one can prove the existence of a subgame-perfect strategy (\ie a $0$-subgame-perfect strategy). 
%\begin{remark}
%  \label{rem:optimal strategies}
%  If $\sigma$ is an optimal strategy then $\reset\sigma$ is subgame-perfect. 
%\end{remark}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

